Actegories for the Working Amthematician

Actions of monoidal categories on categories, also known as actegories, have been familiar to category theorists for a long time, and yet a comprehensive overview of this topic seems to be missing from the literature. Recently, actegories have been increasingly employed in applied category theory, thereby encouraging an effort to fill this gap according to the new needs of these applications. This work started as an investigation of the notion of monoidal actegory, a compatible pair of monoidal and actegorical structures, and ended up including a sizable reference on the elementary theory of actegories. We cover basic definitions and results on actegories and biactegories, spelling out explicitly many folkloric definitions, including their tensor product and their hom-tensor adjunction. We give new definitions of actegories with monoidal, braided monoidal and symmetric monoidal structure. In the last section, we provide three Cayley-like classification results for these structures.

==> src/reflection-structures.tex <==

\subsection{Reflection structures}
We have introduced both balanced and bilinear morphisms of actegories. These are disjoint structures that both deal with `moving scalars around' in a functor, although in different places.
To make the two interact in a nice way, we introduce reflection structures:

\begin{definition}
	Let $\cat C$ be equipped with a left $\cat M$-actegory structure $(\action, \eta^\action, \mu^\action)$ and a right $\cat M$-actegory structure $(\actionn, \eta^\actionn, \mu^\actionn)$.
	A \emph{reflection structure} on $\cat C$ is a morphism $(1, 1, \rho) : (\cat M, \cat C, \action) \longto (\cat M^\rev, \cat C, \actionn)$, that is, a pair of natural morphisms
	\begin{eqalign}
		\beta_{m,n} &: m \mtimes n \longto n \mtimes m,\\
		\rho_{c,n} &: c \actionn m \longto m \action c
	\end{eqalign}
	such that $\beta$ is a monoidal structure for $1_{\cat M}$ and $\rho$ an $\cat M$-linear structure for $1_{\cat C}$. Explicitly, they satisfy the axioms:
	\matteo{$\beta$}
	% https://q.uiver.app/?q=WzAsNixbMiwxLCIobiBcXGFjdGlvbiBjKSBcXGFjdGlvbm4gbSJdLFsxLDAsIihjIFxcYWN0aW9ubiBuKSBcXGFjdGlvbm4gbSJdLFsyLDIsIm0gXFxhY3Rpb24gKG4gXFxhY3Rpb24gYykiXSxbMSwzLCIobSBcXG90aW1lcyBuKSBcXGFjdGlvbiBjIl0sWzAsMSwiYyBcXGFjdGlvbm4gKG4gXFxtdGltZXMgbSkiXSxbMCwyLCJjIFxcYWN0aW9ubiAobSBcXG10aW1lcyBuKSJdLFsxLDAsIlxccmhvX3tjLG59IFxcYWN0aW9ubiBtIl0sWzAsMiwiXFxyaG9fe20sbiBcXGFjdGlvbiBjfSJdLFsyLDMsIlxcbXVeXFxhY3Rpb25fe20sbixjfSJdLFsxLDQsIlxcbXVeXFxhY3Rpb25uX3tjLG4sbX0iLDJdLFs1LDMsIlxccmhvX3tjLCBtXFxtdGltZXMgbn0iLDJdLFs0LDUsImMgXFxhY3Rpb25uIFxcYmV0YV97bixtfSIsMl1d&macro_url=https%3A%2F%2Fgist.githubusercontent.com%2Fmattecapu%2Fb16ea761c7fd7069f7755ccef114985d%2Fraw%2F4fa77ca69b0bb84c9c6d74c93bd1b61b3bfcd6d3%2Factions.sty
	\begin{diagram}
		& {(c \actionn n) \actionn m} \\
		{c \actionn (n \mtimes m)} && {(n \action c) \actionn m} \\
		{c \actionn (m \mtimes n)} && {m \action (n \action c)} \\
		& {(m \otimes n) \action c}
		\arrow["{\rho_{c,n} \actionn m}", from=1-2, to=2-3]
		\arrow["{\rho_{m,n \action c}}", from=2-3, to=3-3]
		\arrow["{\mu^\action_{m,n,c}}", from=3-3, to=4-2]
		\arrow["{\mu^\actionn_{c,n,m}}"', from=1-2, to=2-1]
		\arrow["{\rho_{c, m\mtimes n}}"', from=3-1, to=4-2]
		\arrow["{c \actionn \beta_{n,m}}"', from=2-1, to=3-1]
	\end{diagram}
	% https://q.uiver.app/?q=WzAsMyxbMCwwLCJjIFxcYWN0aW9ubiBqIl0sWzIsMCwiaiBcXGFjdGlvbiBjIl0sWzEsMSwiYyJdLFsyLDAsIlxcZXRhXlxcYWN0aW9ubl9jIl0sWzIsMSwiXFxldGFeXFxhY3Rpb25fYyIsMl0sWzAsMSwiXFxyaG9fe2Msan0iXV0=
	\begin{diagram}
		{c \actionn j} && {j \action c} \\
		& c
		\arrow["{\eta^\actionn_c}", from=2-2, to=1-1]
		\arrow["{\eta^\action_c}"', from=2-2, to=1-3]
		\arrow["{\rho_{c,j}}", from=1-1, to=1-3]
	\end{diagram}
\end{definition}

An actegory equipped with a reflection structure is called a \emph{reflecting actegory}.
Every reflecting actegory is a biactegory with bimodulator given by
\begin{eqalign}
	\zeta_{m,n,c} := m \action (c \actionn n) &\nlongto{m \action \rho_{c,n}} m \action (n \action c)\\
	&\nlongto{\mu^\action_{m,c}} (m \mtimes n) \action c\\
	&\nlongto{\beta_{m,n} \action c} (n \mtimes m) \action c\\
	&\nlongto{{\mu^\actionn_{n}}}
\end{eqalign}

\begin{definition}
	A morphism of reflecting actegories $(\cat C, \action, \rho) \to (\cat D, \actionn, \sigma)$ is a functor $F:\cat C \to \cat D$ such that the following commutes:
	% https://q.uiver.app/?q=WzAsNCxbMCwwLCJGKGMpIFxcYWN0aW9ubiBtIl0sWzEsMCwibSBcXGFjdGlvbiBGKGMpIl0sWzAsMSwiRihjIFxcYWN0aW9ubiBtKSJdLFsxLDEsIkYobSBcXGFjdGlvbiBjKSJdLFswLDEsIlxcc2lnbWFfe0YoYyksbX0iXSxbMCwyLCJcXGVsbF97YyxtfSIsMl0sWzEsMywicl97bSxjfSJdLFsyLDMsIkYoXFxyaG9fe2MsbX0pIiwyXV0=&macro_url=https%3A%2F%2Fgist.githubusercontent.com%2Fmattecapu%2Fb16ea761c7fd7069f7755ccef114985d%2Fraw%2F4fa77ca69b0bb84c9c6d74c93bd1b61b3bfcd6d3%2Factions.sty
	\begin{diagram}
		{F(c) \actionn m} & {m \action F(c)} \\
		{F(c \actionn m)} & {F(m \action c)}
		\arrow["{\sigma_{F(c),m}}", from=1-1, to=1-2]
		\arrow["{\ell_{c,m}}"', from=1-1, to=2-1]
		\arrow["{r_{m,c}}", from=1-2, to=2-2]
		\arrow["{F(\rho_{c,m})}"', from=2-1, to=2-2]
	\end{diagram}
	Equivalently, it is a pair of $\cat M$-linear and $\cat M^\rev$-linear functors $\cat C \to \cat D$ making the obvious square in $\Actt$ commute.
\end{definition}

We have also introduced biactegories, in which two actions can commute past each other.

